Panoramic Image-to-Image Translation

In this paper, we tackle the challenging task of Panoramic Image-to-Image translation (Pano-I2I) for the first time. This task is difficult due to the geometric distortion of panoramic images and the lack of a panoramic image dataset with diverse conditions, like weather or time. To address these challenges, we propose a panoramic distortion-aware I2I model that preserves the structure of the panoramic images while consistently translating their global style referenced from a pinhole image. To mitigate the distortion issue in naive 360 panorama translation, we adopt spherical positional embedding to our transformer encoders, introduce a distortion-free discriminator, and apply sphere-based rotation for augmentation and its ensemble. We also design a content encoder and a style encoder to be deformation-aware to deal with a large domain gap between panoramas and pinhole images, enabling us to work on diverse conditions of pinhole images. In addition, considering the large discrepancy between panoramas and pinhole images, our framework decouples the learning procedure of the panoramic reconstruction stage from the translation stage. We show distinct improvements over existing I2I models in translating the StreetLearn dataset in the daytime into diverse conditions. The code will be publicly available online for our community.

==> tables/detection.tex <==
\begin{table}[ht]
\centering
\setlength{\tabcolsep}{10pt}
% \scalebox{0.8}{
% \small
\begin{tabular}{lc}
\toprule
Methods & {Acc.$\uparrow$} \\ 
\midrule
{CUT} & - \\
{LSeSim} & - \\
{MGUIT}  & -\\
{InstaFormer} & - \\
\midrule
{Ours} & -\\
\bottomrule
\end{tabular}
% }
\caption{\textbf{Results for object detection task.}}
\label{tab:detection}
\end{table}
